High-level Feature Guided Decoding for Semantic Segmentation

Existing pyramid-based upsamplers (e.g. SemanticFPN), although efficient, usually produce less accurate results compared to dilation-based models when using the same backbone. This is partially caused by the contaminated high-level features since they are fused and fine-tuned with noisy low-level features on limited data. To address this issue, we propose to use powerful pre-trained high-level features as guidance (HFG) so that the upsampler can produce robust results. Specifically, \emph{only} the high-level features from the backbone are used to train the class tokens, which are then reused by the upsampler for classification, guiding the upsampler features to more discriminative backbone features. One crucial design of the HFG is to protect the high-level features from being contaminated by using proper stop-gradient operations so that the backbone does not update according to the noisy gradient from the upsampler. To push the upper limit of HFG, we introduce a context augmentation encoder (CAE) that can efficiently and effectively operate on the low-resolution high-level feature, resulting in improved representation and thus better guidance. We named our complete solution as the High-Level Features Guided Decoder (HFGD). We evaluate the proposed HFGD on three benchmarks: Pascal Context, COCOStuff164k, and Cityscapes. HFGD achieves state-of-the-art results among methods that do not use extra training data, demonstrating its effectiveness and generalization ability.

==> tables/ablation_studies_cae_old.tex <==
\begin{table}[t]
\centering
\small
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|l|c|c} 
\toprule
Backbone & Dilated or Upsampler & Extra Encoding & mIOU(\%)  \\
\midrule
\midrule
ResNet-50 & -  &  Identity      &  45.87 \\
ResNet-50 & Dilation, $OS=8$ &  Identity      & \textbf{47.72}  \\
ResNet-50 & SFPN, $OS=4$ &  Identity      & 47.14  \\
\midrule
ResNet-50 & -  & ASPP~\cite{cDeepLabV3Plus}           & 46.41  \\
ResNet-50 & Dilation, $OS=8$  & ASPP~\cite{cDeepLabV3Plus}           & \textbf{48.59}  \\
ResNet-50 & SFPN, $OS=4$ & ASPP~\cite{cDeepLabV3Plus}           &  47.81 \\
\midrule
ResNet-50 & -  & OCR~\cite{cOCR}            & 45.50 \\
ResNet-50 & Dilation, $OS=8$ & OCR~\cite{cOCR}            & \textbf{48.23} \\
ResNet-50 & SFPN, $OS=4$ & OCR~\cite{cOCR}            & 47.39 \\
\midrule
ResNet-50 & - & SA~\cite{cNonLocal} & 45.02 \\
ResNet-50 & Dilation, $OS=8$ & SA~\cite{cNonLocal} & \textbf{48.32} \\
ResNet-50 & SFPN, $OS=4$ & SA~\cite{cNonLocal} & 45.90 \\
\midrule
ResNet-50 & - & SA~(CAR~\cite{cCAR}) &  47.18  \\
ResNet-50 & Dilation, $OS=8$ & SA~(CAR~\cite{cCAR}) & \textbf{50.50} \\
ResNet-50 & SFPN, $OS=4$ & SA~(CAR~\cite{cCAR}) & 48.51  \\
\midrule
ResNet-50 & - & Our CAE  & 47.35 \\
ResNet-50 & Dilation, $OS=8$ & Our CAE  & \textbf{49.67} \\
ResNet-50 & SFPN, $OS=4$ & Our CAE  & 48.76 \\
\bottomrule
\end{tabular}
}
\caption{
% Experiments to compare the effectiveness of using dilated backbones and upsampler networks on Pascal Context dataset.
\dk{
Effectiveness comparisons on Pascal Context dataset.
}
Using a dilated backbone consistently outperforms using an upsampler net on several representative context encoding methods.
% of different encoding modules for high-level feature enhancements on Pascal Context dataset.
% 
The final feature maps are bilinearly upsampled to the image resolution \dk{right before} the class label prediction.
% We train all the methods under exactly same and fair settings.
%
% Experiments without upsampling head produces $OS=32$ feature maps while those with Semantic FPN (SFPN)~\cite{cPanopticFPN} produces $OS=4$ feature maps.
}
\label{tab:ablation_cae}
\end{table}
